Decodable and Sample Invariant Continuous Object Encoder

We propose Hyper-Dimensional Function Encoding (HDFE). Given samples of a continuous object (e.g. a function), HDFE produces an explicit vector representation of the given object, invariant to the sample distribution and density. Sample distribution and density invariance enables HDFE to consistently encode continuous objects regardless of their sampling, and therefore allows neural networks to receive continuous objects as inputs for machine learning tasks, such as classification and regression. Besides, HDFE does not require any training and is proved to map the object into an organized embedding space, which facilitates the training of the downstream tasks. In addition, the encoding is decodable, which enables neural networks to regress continuous objects by regressing their encodings. Therefore, HDFE serves as an interface for processing continuous objects. We apply HDFE to function-to-function mapping, where vanilla HDFE achieves competitive performance as the state-of-the-art algorithm. We apply HDFE to point cloud surface normal estimation, where a simple replacement from PointNet to HDFE leads to immediate 12% and 15% error reductions in two benchmarks. In addition, by integrating HDFE into the PointNet-based SOTA network, we improve the SOTA baseline by 2.5% and 1.7% in the same benchmarks.

==> src/app4_iterative_refinement.tex <==
In the iterative refinement section, we claim that the iterative refinement (Algorithm \ref{alg:1}) will converge to \textit{the center of the smallest ball containing all the sample encodings}. In this section, we detail the proof of the argument.
\newpage

==> src/s21_VFA.tex <==
\textbf{VFA} \citep{frady2021computing}. A function of the form $\mathfrak{h}(x)=\sum_{k}\alpha_k\cdot K(x,x_k)$ is represented by $\V_\mathfrak{h}=\sum_k \alpha_k\cdot E(x_k)$, where the kernel $K:\mathbb{C}^N\times\mathbb{C}^N\rightarrow \mathbb{R}$ and the encoder $E:X\rightarrow \mathbb{C}^N$ satisfy $K(x-y)=\langle E(x), E(y) \rangle$.

VFA can encode an explicit function into a fixed-length vector, where the encoding is sample invariant and decodable. However, VFA assumes the function satisfies the functional form $\mathfrak{h}(x)$, which can easily fail. A naive example is the constant function $f(x)=1$. To approximate the constant function, the kernel $K$ must be constant $K(x,y)=c$. Clearly, with such selection of $K$, $\mathfrak{h}(x)$ cannot approximate other non-constant functions. In addition, \citet{frady2021computing} only provides empirical evaluation without real-world applications.

In this paper, HDFE relaxes the strong assumption required by VFA and enables encoding Lipschitz functions. Since the strong assumption is relaxed, we apply HDFE to two real-world applications. In the Appendix \ref{sec:app_VFA}, we show a non-trivial example where VFA fails to reconstruct the function while HDFE succeeds. We also provide more detailed comparison between VFA and HDFE.


==> src/s99_PDE_quali.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-28pt}
\begin{minipage}{0.5\textwidth}
\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/PDE_qualitative/input.jpeg}
         % \caption{Input function.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/PDE_qualitative/GT.jpeg}
         % \caption{Ground-truth solution.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/PDE_qualitative/pred.jpeg}
         % \caption{Predicted solution.}
     \end{subfigure}
        \caption{Qualitative results for Darcy flow predicted by HDFE. \textbf{Left}: Input function. \textbf{Mid}: Ground-truth solution. \textbf{Right}: Predicted solution.}
        \label{fig:fig5}
\end{figure}
\end{minipage}
\vspace{-7pt}
\end{wrapfigure}



